In-Context Example Selection via Similarity Search Improves Low-Resource Machine Translation

The ability of generative large language models (LLMs) to perform in-context learning has given rise to a large body of research into how best to prompt models for various natural language processing tasks. In this paper, we focus on machine translation (MT), a task that has been shown to benefit from in-context translation examples. However no systematic studies have been published on how best to select examples, and mixed results have been reported on the usefulness of similarity-based selection over random selection. We provide a study covering multiple LLMs and multiple in-context example retrieval strategies, comparing multilingual sentence embeddings. We cover several language directions, representing different levels of language resourcedness (English into French, German, Swahili and Wolof). Contrarily to previously published results, we find that sentence embedding similarity can improve MT, especially for low-resource language directions, and discuss the balance between selection pool diversity and quality. We also highlight potential problems with the evaluation of LLM-based MT and suggest a more appropriate evaluation protocol, adapting the COMET metric to the evaluation of LLMs. Code and outputs are freely available at https://github.com/ArmelRandy/ICL-MT.

==> garbage.tex <==
% BLEU 5

\begin{table*}[ht]
%\tiny
\centering\small
\begin{center}
%\resizebox{0.5\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
\toprule
\multicolumn{1}{c}{\bf }  & \multicolumn{3}{c}{\bf eng $\rightarrow$ fra} & \multicolumn{3}{c}{\bf eng $\rightarrow$ deu} & \multicolumn{3}{c}{\bf eng $\rightarrow$ swh} & \multicolumn{3}{c}{\bf eng $\rightarrow$ wol}\\
 {} & 1 & 5 & 10 & 1 & 5 & 10 & 1 & 5 & 10 & 1 & 5 & 10\\
\midrule
Gemma~2B \\
\midrule
Embed v3 & 42.0 & 43.4 & 43.9 & 31.8 & 33.4 & 33.6 & 11.4 & \bf 14.1 & \bf 14.7 & 2.2 & 2.7 & 3.0 \\
E5 & 42.4 & 43.4 & \bf 44.1 & 32.3 & 33.4 & 33.9 & 11.1 & 13.9 & 14.5 & 2.2 & 2.5 & 2.7 \\
LaBSE & 42.5 & 43.3 & 44.1 & \bf 32.5 & 33.2 & 33.7 & 11.4 & 13.7 & 14.5 & 2.4 & 2.7 & 3.0 \\
LASER2 & 42.3 & 43.4 & 43.9 & 32.2 & 33.2 & 33.9 & 11.1 & 13.4 & 13.8 & 2.4 & 2.5 & 2.7 \\
SONAR & \bf 42.9 & \bf 43.7 & 44.0 & 32.4 & \bf 33.7 & \bf 34.0 & \bf 11.4 & 13.7 & 14.5 & \bf 2.6 & \bf 2.8 & \bf 3.2 \\
Random & 42.2 & 42.8 & 43.3 & 31.7 & 32.8 & 33.2 & 10.7 & 12.0 & 12.6 & 1.2 & 1.5 & 1.7 \\
\midrule
OLMo~7B \\
\midrule
Embed v3 & \bf 35.1 & 35.8 & 36.0 & 23.4 & 23.9 & 23.6 & 3.2 & 4.1 & 4.2 & 2.3 & 2.5 & 2.6 \\
E5 & 35.1 & 35.7 & 35.9 & 23.3 & \bf 24.1 & \bf 23.9 & 3.2 & 3.8 & 4.1 & 2.3 & 2.4 & 2.5 \\
LaBSE & 35.0 & 35.6 & \bf 36.5 & 23.6 & 23.5 & 23.7 & 3.5 & 4.0 & 4.2 & 2.5 & 2.5 & 2.7 \\
LASER2 & 35.0 & 35.6 & 35.7 & 23.2 & 23.5 & 23.6 & 2.9 & 3.7 & 3.9 & 2.5 & 2.6 & 2.8 \\
SONAR & 34.9 & \bf 35.9 & 36.2 & \bf 23.8 & 23.3 & 23.1 & \bf 3.4 & \bf 4.4 & \bf 4.5 & \bf 2.6 & \bf 2.6 & \bf 2.9 \\
Random & 34.9 & 35.0 & 34.9 & 22.7 & 22.9 & 22.8 & 2.3 & 2.6 & 2.6 & 1.5 & 1.5 & 1.7 \\
\midrule
LLaMA 2 13B \\
\midrule
Embed v3 & 48.6 & 49.7 & 49.9 & 38.5 & 38.9 & 39.5 & 4.4 & \bf 6.0 & 6.4 & 2.4 & 3.0 & 3.1 \\
E5 & 48.8 & 49.6 & 50.1 & \bf 38.6 & \bf 39.5 & \bf 39.7 & 4.3 & 5.7 & 6.1 & 2.3 & 3.0 & 3.0 \\
LaBSE & 48.4 & \bf 50.2 & 50.2 & 38.2 & 39.5 & 39.7 & 4.3 & 5.8 & 6.3 & 2.7 & 3.0 & 3.4 \\
LASER2 & 48.8 & 49.9 & \bf 50.4 & 38.5 & 39.4 & 39.6 & 4.4 & 5.4 & 5.9 & 2.6 & 3.1 & \bf 3.4 \\
SONAR & \bf 49.1 & 49.9 & 50.2 & 38.5 & 39.0 & 39.6 & \bf 4.5 & 5.7 & \bf 6.7 & \bf 2.6 & \bf 3.2 & 3.3 \\
Random & 48.7 & 49.6 & 50.2 & 38.0 & 39.0 & 39.4 & 3.8 & 4.3 & 4.5 & 1.7 & 2.0 & 2.2 \\
\midrule
LLaMA 2 70B \\
\midrule
Embed v3 & 52.6 & 53.5 & 53.9 & 43.3 & 44.0 & \bf 44.5 & \bf 8.8 & \bf 11.5 & 12.0 & 2.5 & 3.3 & 3.8 \\
E5 & 52.7 & 53.7 & 54.2 & 43.3 & 44.0 & 44.5 & 8.7 & 11.6 & 12.1 & 2.6 & 3.4 & 3.6 \\
LaBSE & \bf 53.0 & 53.8 & 53.9 & 43.0 & 43.9 & 44.2 & 8.8 & 11.7 & 12.3 & \bf 3.1 & 3.5 & 3.8 \\
LASER2 & 52.9 & \bf 54.0 & \bf 54.5 & 43.1 & 43.8 & 43.9 & 8.6 & 10.7 & 11.4 & 2.9 & 3.4 & 3.8 \\
SONAR & 52.8 & 53.7 & 54.3 & \bf 43.4 & \bf 44.4 & 44.4 & 8.7 & 11.4 & \bf 12.6 & 2.8 & \bf 3.6 & \bf 3.8 \\
Random & 52.5 & 53.5 & 53.9 & 43.1 & 43.6 & 43.8 & 7.6 & 9.3 & 9.6 & 2.1 & 2.4 & 2.6 \\
\midrule
Mixtral~8x7B~v0.1 \\
\midrule
Embed v3 & 54.3 & 54.8 & 55.1 & 44.2 & 44.8 & 45.3 & 7.5 & \bf 9.4 & \bf 10.7 & 2.5 & \bf 3.4 & 3.5 \\
E5 & 53.9 & \bf 55.1 & \bf 55.4 & 44.1 & \bf 45.3 & \bf 45.6 & \bf 7.7 & 9.1 & 9.9 & 2.5 & 3.3 & 3.3 \\
LaBSE & \bf 54.6 & 55.0 & 55.2 & 43.9 & 45.0 & 44.9 & 7.4 & 9.2 & 10.5 & 2.8 & 3.1 & 3.6 \\
LASER2 & 54.5 & 55.0 & 55.3 & \bf 44.4 & 45.1 & 44.8 & 7.0 & 9.0 & 9.6 & 2.7 & 3.3 & 3.4 \\
SONAR & 54.5 & 54.9 & 55.3 & 43.7 & 45.0 & 45.3 & 7.5 & 9.2 & 10.3 & \bf 2.8 & 3.3 & \bf 3.6 \\
Random & 54.1 & 54.6 & 54.9 & 43.8 & 44.6 & 44.9 & 6.5 & 7.0 & 7.5 & 1.9 & 2.2 & 2.5 \\
\bottomrule
\end{tabular}
%}
\end{center}
\caption{Additional results (with other LLMs): BLEU results for example retrieval with different sentence embeddings in $k$-shot settings ($k \in \{1, 5, 10\}$).}
\label{tab:more-bleu-se}
\end{table*}



% COMET 5

\begin{table*}[ht]
%\tiny
\centering\small
\begin{center}
%\resizebox{0.5\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
\toprule
\multicolumn{1}{c}{\bf }  & \multicolumn{3}{c}{\bf eng $\rightarrow$ fra} & \multicolumn{3}{c}{\bf eng $\rightarrow$ deu} & \multicolumn{3}{c}{\bf eng $\rightarrow$ swh} & \multicolumn{3}{c}{\bf eng $\rightarrow$ wol}\\
 {} & 1 & 5 & 10 & 1 & 5 & 10 & 1 & 5 & 10 & 1 & 5 & 10\\
\midrule
Gemma~2B \\
\midrule
Embed v3 & 84.7 & 85.3 & \bf 85.4 & 82.6 & 83.1 & 83.3 & 64.9 & \bf 68.5 & 69.0 & \bf 45.6 & \bf 47.7 & 48.7 \\
E5 & 84.6 & 85.1 & \bf 85.4 & \bf 82.8 & 83.2 & 83.3 & 64.9 & 68.2 & 68.5 & 45.4 & 47.4 & 48.3 \\
LaBSE & \bf 84.8 & \bf 85.2 & \bf 85.4 & 82.7 & \bf 83.4 & 83.4 & \bf 65.2 & 67.6 & 68.5 & 43.9 & 47.0 & 48.4 \\
LASER2 & 84.6 & 85.0 & 85.0 & 82.7 & 83.2 & 83.2 & 64.5 & 67.1 & 67.8 & 42.2 & 45.3 & 46.4 \\
SONAR & \bf 84.8 & \bf 85.2 & 85.3 & 82.6 & 83.2 & \bf 83.5 & 64.9 & 67.9 & \bf 69.1 & 45.1 & 46.7 & \bf 48.9 \\
Random & 84.6 & 84.7 & 85.0 & 82.3 & 82.9 & 83.1 & 63.6 & 65.3 & 65.8 & 38.2 & 39.3 & 40.4 \\
\midrule
OLMo~7B \\
\midrule
Embed v3 & 81.1 & 81.2 & 81.3 & \bf 75.6 & 76.0 & 75.8 & 44.5 & 43.9 & 44.8 & \bf 46.6 & \bf 45.1 & 45.8 \\
E5 & 81.1 & 81.4 & 81.4 & 75.3 & 76.2 & \bf 76.3 & 44.2 & 43.1 & 44.0 & 46.5 & 44.7 & 45.7 \\
LaBSE & \bf 81.2 & 81.4 & 81.5 & 75.3 & 76.0 & 76.1 & 44.3 & 43.5 & 44.1 & 45.5 & 44.7 & 45.8 \\
LASER2 & 81.0 & \bf 81.5 & \bf 81.5 & 75.0 & \bf 76.4 & \bf 76.3 & 41.5 & 41.3 & 42.2 & 44.1 & 43.7 & 44.7 \\
SONAR & 81.1 & 81.3 & 81.3 & 75.5 & 76.2 & 76.1 & \bf 44.7 & \bf 44.3 & \bf 45.1 & 46.1 & 44.9 & \bf 46.8 \\
Random & 81.1 & 81.0 & 80.9 & 75.1 & 75.7 & 75.6 & 38.3 & 38.4 & 38.4 & 39.9 & 38.7 & 40.1 \\
\midrule
LLaMA 2 13B \\
\midrule
Embed v3 & 87.2 & 87.3 & \bf 87.6 & 86.1 & 86.1 & 86.5 & \bf 46.0 & 48.2 & \bf 49.4 & 47.4 & 46.2 & 47.0 \\
E5 & 87.1 & 87.3 & 87.5 & \bf 86.2 & 86.4 & 86.5 & 46.0 & 48.0 & 49.0 & \bf 47.9 & 46.9 & 46.8 \\
LaBSE & \bf 87.2 & \bf 87.4 & 87.4 & 85.9 & \bf 86.5 & 86.7 & 44.9 & 47.6 & 48.9 & 46.7 & 46.1 & 46.3 \\
LASER2 & 87.1 & 87.3 & 87.4 & 86.0 & 86.4 & 86.5 & 44.3 & 46.0 & 47.1 & 44.8 & 45.6 & 45.9 \\
SONAR & 87.2 & 87.2 & 87.4 & 85.9 & 86.2 & \bf 86.8 & 45.6 & \bf 48.3 & \bf 49.4 & 46.7 & \bf 47.4 & \bf 47.0 \\
Random & 87.0 & 87.2 & 87.4 & 85.9 & 86.1 & 86.4 & 41.8 & 42.6 & 43.1 & 40.0 & 40.0 & 40.7 \\
\midrule
LLaMA 2 70B \\
\midrule
Embed v3 & 87.7 & 88.2 & 88.2 & \bf 87.3 & 87.7 & \bf 87.9 & 56.4 & \bf 61.4 & 62.8 & 46.3 & 49.4 & \bf 50.8 \\
E5 & \bf 87.9 & 88.1 & \bf 88.4 & \bf 87.3 & 87.7 & \bf 87.9 & 56.2 & 61.3 &  \bf 63.1 & \bf 46.6 & \bf 50.0 & 49.7 \\
LaBSE & 87.7 & \bf 88.2 & 88.3 & 87.1 & \bf 87.8 & \bf 87.9 & \bf 56.6 & 60.9 & 62.5 & 46.2 & 49.9 & 49.9 \\
LASER2 & 87.7 & \bf 88.2 & 88.3 & \bf 87.3 & 87.6 & 87.8 & 55.9 & 59.7 & 60.9 & 45.2 & 48.9 & 49.6 \\
SONAR & \bf 87.9 & \bf 88.2 & 88.3 & \bf 87.3 & \bf 87.8 & 87.8 & 56.2 & 61.0 & 62.8 & 46.3 & 49.9 & 50.2 \\
Random & 87.6 & 88.0 & 88.1 & 87.2 & 87.5 & 87.7 & 53.5 & 56.8 & 57.6 & 41.0 & 43.0 & 44.0 \\
\midrule
Mixtral~8x7B~v0.1 \\
\midrule
Embed v3 & \bf 88.2 & 88.4 & \bf 88.5 & 87.8 & 87.9 & 88.2 & 54.9 & 57.8 & \bf 60.4 & 43.6 & 48.5 & 50.0 \\
E5 & 88.1 & \bf 88.5 & 88.4 & 87.7 & \bf 88.2 & \bf 88.3 & \bf 55.2 & 57.6 & 59.9 & \bf 43.9 & \bf 48.6 & 50.0 \\
LaBSE & \bf 88.2 & 88.4 & \bf 88.5 & \bf 87.9 & 88.1 & 88.1 & 55.0 & 57.6 & 59.2 & 43.3 & 48.5 & \bf 50.3 \\
LASER2 & 88.1 & 88.4 & 88.4 & 87.7 & \bf 88.2 & 88.0 & 53.4 & 56.5 & 58.3 & 42.7 & 48.0 & 49.5 \\
SONAR & \bf 88.2 & 88.4 & \bf 88.5 & 87.5 & 88.0 & \bf 88.3 & 55.1 & \bf 58.0 & 59.3 & 43.4 & 48.3 & 50.1 \\
Random & 88.1 & 88.3 & 88.4 & 87.6 & 88.0 & 88.1 & 52.5 & 53.5 & 54.4 & 38.7 & 42.6 & 44.6 \\
\bottomrule
\end{tabular}
%}
\end{center}
\caption{Additional results (other LLMs): COMET results for example retrieval with different sentence embeddings in $k$-shot settings ($k \in \{1, 5, 10\}$).}
\label{tab:more-comet-se}
\end{table*}


% BLEU 5 comparison
\begin{table*}[ht]
%\tiny
\centering\small
\begin{center}
%\resizebox{0.5\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
\toprule
\multicolumn{1}{c}{\bf }  & \multicolumn{3}{c}{\bf eng $\rightarrow$ fra} & \multicolumn{3}{c}{\bf eng $\rightarrow$ deu} & \multicolumn{3}{c}{\bf eng $\rightarrow$ swh} & \multicolumn{3}{c}{\bf eng $\rightarrow$ wol}\\
 {} & 1 & 5 & 10 & 1 & 5 & 10 & 1 & 5 & 10 & 1 & 5 & 10\\
\midrule
Gemma~2B \\
\midrule
SONAR & \bf 42.9 & 43.7 & 44.0 & \bf 32.4 & \bf 33.7 & \bf 34.0 & 11.4 & 13.7 & 14.5 & \bf 2.6 & \bf 2.8 & \bf 3.2\\
BM25 & 42.7 & \bf 43.9 & \bf 44.3 & 31.9 & 33.5 & 33.4 & 11.9 & \bf 14.3 & \bf 15.1 & 1.8 & 2.3 & 2.6 \\
R-BM25 & 42.2 & 42.9 & 42.9 & 31.4 & 32.7 & 32.9 & 11.0 & 11.9 & 12.0 & 1.7 & 1.5 & 1.8 \\
BLEU & 42.7 & 43.5 & 43.9 & 32.0 & 33.5 & 33.6 & \bf 12.1 & 14.1 & 14.3 & 2.0 & 2.1 & 2.6 \\
RoBERTa & 42.6 & 43.4 & 43.6 & 31.7 & 33.5 & 33.5 & 11.0 & 12.7 & 12.8 & 1.7 & 1.9 & 2.1 \\
Random & 42.2 & 42.8 & 43.3 & 31.7 & 32.8 & 33.2 & 10.7 & 12.0 & 12.6 & 1.2 & 1.5 & 1.7 \\
\midrule
OLMo~7B \\
\midrule
SONAR & 34.9 & 35.9 & \bf 36.2 & \bf 23.8 & 23.3 & 23.1 & \bf 3.4 & \bf 4.4 & \bf 4.5 & \bf 2.6 & \bf 2.6 & \bf 2.9 \\
BM25 & 35.1 & 36.0 & 36.1 & 23.0 & 23.4 & 23.5 & 3.4 & 4.0 & 4.3 & 2.3 & 2.2 & 2.5 \\
R-BM25 & 34.6 & 35.1 & 35.3 & 23.0 & 22.6 & 22.8 & 2.4 & 2.6 & 2.7 & 1.5 & 1.8 & 1.8 \\
BLEU & \bf 35.5 & \bf 36.0 & 36.1 & 23.0 & \bf 23.7 & \bf 23.6 & 3.2 & 3.8 & 4.3 & 1.9 & 2.2 & 2.3 \\
RoBERTa & 35.0 & 35.3 & 35.3 & 23.2 & 23.3 & 23.4 & 3.0 & 2.9 & 3.2 & 1.8 & 1.8 & 1.8 \\
Random & 34.9 & 35.0 & 34.9 & 22.7 & 22.9 & 22.8 & 2.3 & 2.6 & 2.6 & 1.5 & 1.5 & 1.7 \\
\midrule
LLaMA 2 13B \\
\midrule
SONAR & \bf 49.1 & \bf 49.9 & 50.2 & 38.5 & 39.0 & 39.6 & 4.5 & 5.7 & \bf 6.7 & \bf 2.6 & \bf 3.2 & \bf 3.3 \\
BM25 & 48.8 & 49.4 & 50.2 & \bf 38.6 & \bf 39.3 & \bf 39.9 & 4.5 & \bf 6.0 & 6.6 & 2.2 & 2.9 & 3.2 \\
R-BM25 & 49.0 & 49.4 & 50.1 & 37.7 & 38.7 & 39.2 & 3.8 & 4.2 & 4.5 & 1.7 & 2.0 & 2.2 \\
BLEU & \bf 49.1 & 49.7 & \bf 50.4 & 38.3 & 39.1 & 39.7 & \bf 4.6 & 5.7 & 6.4 & 2.1 & 2.7 & 3.0 \\
RoBERTa & 48.3 & 49.5 & 50.2 & 38.2 & 38.9 & 39.4 & 3.9 & 4.7 & 5.3 & 1.8 & 2.4 & 2.6 \\
Random & 48.7 & 49.6 & 50.2 & 38.0 & 39.0 & 39.4 & 3.8 & 4.3 & 4.5 & 1.7 & 2.0 & 2.2 \\
\midrule
LLaMA 2 70B \\
\midrule
SONAR & \bf 52.8 & 53.7 & \bf 54.3 & \bf 43.4 & \bf 44.4 & \bf 44.4 & \bf 8.7 & 11.4 & 12.6 & \bf 2.8 & \bf 3.6 & \bf 3.8 \\
BM25 & 52.8 & 53.5 & 54.2 & 42.9 & 43.6 & 44.0 & 8.6 & \bf 12.0 & \bf 12.9 & 2.6 & 3.1 & 3.7 \\
R-BM25 & 52.4 & 53.4 & 53.8 & 42.9 & 43.9 & 43.6 & 7.3 & 9.1 & 9.8 & 1.9 & 2.4 & 2.6 \\
BLEU & 52.5 & \bf 53.8 & 54.0 & 42.8 & 43.7 & 44.1 & 8.5 & 11.4 & 11.9 & 2.5 & 3.0 & 3.4 \\
RoBERTa & 52.3 & 53.1 & 53.8 & 43.2 & 43.6 & 44.0 & 8.2 & 9.9 & 10.5 & 2.2 & 2.7 & 2.8 \\
Random & 52.5 & 53.5 & 53.9 & 43.1 & 43.6 & 43.8 & 7.6 & 9.3 & 9.6 & 2.1 & 2.4 & 2.6 \\
\midrule
Mixtral~8x7B~v0.1 \\
\midrule
SONAR & \bf 54.5 & \bf 54.9 & \bf 55.3 & 43.7 & \bf 45.0 & \bf 45.3 & 7.5 & 9.2 & 10.3 & \bf 2.8 & \bf 3.3 & \bf 3.6 \\
BM25 & 53.9 & 54.6 & 54.6 & 44.0 & 44.7 & 44.9 & \bf 7.6 & \bf 9.7 & \bf 10.7 & 2.3 & 3.2 & 3.4 \\
R-BM25 & 54.0 & 54.8 & 54.5 & \bf 44.1 & 44.3 & 44.3 & 6.5 & 6.9 & 7.4 & 2.0 & 2.4 & 2.4 \\
BLEU & 53.7 & \bf 54.9 & 54.8 & 44.0 & 44.6 & 44.5 & 7.4 & 9.2 & 9.9 & 2.2 & 2.9 & 3.3 \\
RoBERTa & 54.3 & \bf 54.9 & \bf 55.3 & \bf 44.1 & 44.8 & 44.9 & 7.0 & 7.8 & 8.4 & 2.1 & 2.7 & 2.9 \\
Random & 54.1 & 54.6 & 54.9 & 43.8 & 44.6 & 44.9 & 6.5 & 7.0 & 7.5 & 1.9 & 2.2 & 2.5 \\
\bottomrule
\end{tabular}
%}
\end{center}
\caption{Comparison of example retrieval with SONAR to baseline methods in $k$-shot ($k \in \{1, 5, 10\}$). We report the BLEU scores for 5 LLMs.}
\label{tab:more-bleu-comparison}
\end{table*}

% COMET 5 comparison
\begin{table*}[ht]
%\tiny
\centering\small
\begin{center}
%\resizebox{0.5\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
\toprule
\multicolumn{1}{c}{\bf }  & \multicolumn{3}{c}{\bf eng $\rightarrow$ fra} & \multicolumn{3}{c}{\bf eng $\rightarrow$ deu} & \multicolumn{3}{c}{\bf eng $\rightarrow$ swh} & \multicolumn{3}{c}{\bf eng $\rightarrow$ wol}\\
 {} & 1 & 5 & 10 & 1 & 5 & 10 & 1 & 5 & 10 & 1 & 5 & 10\\
\midrule
Gemma~2B \\
\midrule
SONAR &\bf 84.8 & \bf 85.2 & \bf 85.3 & \bf 82.6 & 83.2 & \bf 83.5 & 64.9 & \bf 67.9 & \bf 69.1 & \bf 45.1 & \bf 46.7 & \bf 48.9 \\
BM25 & 84.7 & 85.1 & 85.2 & \bf 82.6 & 83.0 & 83.1 & \bf 65.2 & 67.7 & 68.7 & 43.3 & 45.4 & 46.7 \\
R-BM25 & 84.6 & 84.9 & 84.8 & 82.5 & 83.2 & 83.1 & 64.1 & 65.2 & 65.7 & 37.1 & 37.9 & 39.0 \\
BLEU & \bf 84.8 & 85.1 & 85.1 & 82.4 & 83.2 & 83.0 & 64.8 & 67.4 & 67.4 & 42.2 & 44.1 & 45.1 \\
RoBERTa & \bf 84.8 & 85.0 & 85.0 & 82.3 & \bf 83.3 & \bf 83.5 & 64.1 & 66.5 & 66.6 & 41.7 & 43.2 & 44.8 \\
Random & 84.6 & 84.7 & 85.0 & 82.3 & 82.9 & 83.1 & 63.6 & 65.3 & 65.8 & 38.2 & 39.3 & 40.4 \\
\midrule
OLMo~7B \\
\midrule
SONAR & \bf 81.1 & 81.3 & \bf 81.3 & 75.5 & \bf 76.2 & \bf 76.1 & \bf 44.7 & \bf 44.3 & \bf 45.1 & \bf 46.1 & \bf 44.9 & \bf 46.8 \\
BM25 & 80.9 & \bf 81.4 & 81.1 & 75.2 & 75.8 & 75.9 & 42.5 & 42.1 & 43.0 & 43.9 & 43.7 & 45.1 \\
R-BM25 & 80.5 & 80.9 & 80.9 & 75.5 & 75.5 & 75.5 & 38.0 & 38.2 & 38.7 & 37.8 & 37.6 & 39.4 \\
BLEU & 81.0 & 81.2 & 81.1 & \bf 75.6 & 75.6 & 75.8 & 41.4 & 41.4 & 42.0 & 43.0 & 43.3 & 44.6 \\
RoBERTa & \bf 81.1 & 81.2 & 81.0 & 75.1 & 75.9 & 75.5 & 41.0 & 40.0 & 40.5 & 43.4 & 41.5 & 42.0 \\
Random & \bf 81.1 & 81.0 & 80.9 & 75.1 & 75.7 & 75.6 & 38.3 & 38.4 & 38.4 & 39.9 & 38.7 & 40.1 \\
\midrule
LLaMA 2 13B \\
\midrule
SONAR & \bf 87.2 & \bf 87.2 & 87.4 & 85.9 & 86.2 & \bf 86.8 & \bf 45.6 & \bf 48.3 & \bf 49.4 & \bf 46.7 & \bf 47.4 & \bf 47.0 \\
BM25 & 86.9 & 87.1 & 87.4 & \bf 86.2 & 86.1 & 86.6 & 44.1 & 46.8 & 48.0 & 45.2 & 45.6 & 46.8 \\
R-BM25 & 87.1 & \bf 87.2 & 87.3 & \bf 86.2 & \bf 86.3 & 86.5 & 42.0 & 41.8 & 42.6 & 39.4 & 39.7 & 40.3 \\
BLEU & 87.0 & 86.6 & 87.4 & 86.0 & 85.9 & 86.6 & 43.5 & 45.7 & 46.6 & 44.3 & 45.3 & 45.5 \\
RoBERTa & 87.0 & 87.0 & \bf 87.5 & 86.1 & 86.0 & 86.5 & 42.8 & 44.1 & 45.2 & 44.6 & 43.3 & 43.3 \\
Random & 87.0 & 87.2 & 87.4 & 85.9 & 86.1 & 86.4 & 41.8 & 42.6 & 43.1 & 40.0 & 40.0 & 40.7 \\
\midrule
LLaMA 2 70B \\
\midrule
SONAR & \bf 87.9 & \bf 88.2 & \bf 88.3 & \bf 87.3 & \bf 87.8 & \bf 87.8 & \bf 56.2 & \bf 61.0 & \bf 62.8 & \bf 46.3 & \bf 49.9 & \bf 50.2 \\
BM25 & 87.8 & 88.0 & 88.2 & 87.0 & 87.6 & \bf 87.8 & 54.7 & 60.4 & 61.9 & 44.7 & 47.9 & 49.7 \\
R-BM25 & 87.7 & 88.0 & 88.1 & 87.2 & 87.6 & 87.7 & 52.8 & 56.3 & 57.8 & 38.1 & 42.0 & 44.2 \\
BLEU & 87.6 & 88.0 & 88.2 & 87.2 & 87.5 & 87.7 & 54.6 & 59.6 & 60.3 & 44.1 & 47.6 & 48.2 \\
RoBERTa & 87.7 & 88.0 & 88.2 & 87.3 & 87.6 & 87.7 & 54.8 & 58.2 & 59.1 & 44.5 & 46.5 & 47.0 \\
Random & 87.6 & 88.0 & 88.1 & 87.2 & 87.5 & 87.7 & 53.5 & 56.8 & 57.6 & 41.0 & 43.0 & 44.0 \\
\midrule
Mixtral~8x7B~v0.1 \\
\midrule
SONAR & \bf 88.2 & 88.4 & \bf 88.5 & 87.5 & \bf 88.0 & \bf 88.3 & \bf 55.1 & \bf 58.0 & \bf 59.3 & \bf 43.4 & \bf 48.3 & \bf 50.1 \\
BM25 & 88.0 & 88.3 & 88.3 & \bf 87.7 & 88.0 & 88.1 & 54.6 & 57.6 & 58.7 & 42.0 & 48.3 & 49.4 \\
R-BM25 & 88.1 & 88.3 & 88.3 & 87.6 & 87.9 & 88.0 & 52.6 & 53.9 & 54.8 & 37.3 & 40.7 & 42.6 \\
BLEU & 87.9 & 88.4 & 88.4 & 87.6 & 88.0 & 88.1 & 53.9 & 56.9 & 57.6 & 41.5 & 46.9 & 48.7 \\
RoBERTa & 88.1 & \bf 88.5 & 88.5 & 87.6 & 87.9 & 88.0 & 53.8 & 55.2 & 55.9 & 41.7 & 45.3 & 47.6 \\
Random & 88.1 & 88.3 & 88.4 & 87.6 & 88.0 & 88.1 & 52.5 & 53.5 & 54.4 & 38.7 & 42.6 & 44.6 \\
\bottomrule
\end{tabular}
%}
\end{center}
\caption{Comparison of example retrieval with SONAR to baseline methods in $k$-shot ($k \in \{1, 5, 10\}$). We report the COMET scores for 5 LLMs.}
\label{tab:more-comet-comparison}
\end{table*}

\section{s2t}

\begin{table*}[ht]
%\tiny
\centering\small
\begin{center}
%\resizebox{0.5\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
\toprule
\multicolumn{1}{c}{\bf }  & \multicolumn{3}{c}{\bf eng $\rightarrow$ fra} & \multicolumn{3}{c}{\bf eng $\rightarrow$ deu} & \multicolumn{3}{c}{\bf eng $\rightarrow$ swh} & \multicolumn{3}{c}{\bf eng $\rightarrow$ wol}\\
 {} & 1 & 5 & 10 & 1 & 5 & 10 & 1 & 5 & 10 & 1 & 5 & 10\\
\midrule
BLOOM~7B1 \\
\midrule
Embed v3 & \bf 42.7 & 47.4 & 47.7 & 12.5 & 14.9 & 15.0 & 8.6 & 11.7 & 12.1 & 2.0 & 2.7 & 2.7 \\
E5 & 42.6 & 47.2 & 47.7 & 12.2 & 14.6 & 14.8 & 8.9 & 11.2 & 12.3 & 1.5 & 2.4 & 2.5 \\
LaBSE & 42.5 & 47.5 & 48.0 & 12.6 & 14.9 & 15.3 & 8.6 & \bf 11.8 & 12.0 & 2.2 & 2.6 & 2.8 \\
LASER2 & 41.9 & \bf 47.8 & \bf 48.0 & \bf 12.7 & \bf 15.1 & 15.1 & \bf 8.9 & 11.2 & 11.8 & 2.0 & 2.6 & 2.6 \\
SONAR & 42.5 & 47.2 & 47.6 & 12.7 & 14.9 & \bf 15.3 & 8.2 & 11.6 & \bf 12.5 & \bf 2.4 & \bf 2.9 & \bf 3.1 \\
Random & 40.8 & 46.7 & 47.2 & 12.3 & 13.9 & 14.0 & 8.2 & 10.5 & 11.0 & 0.9 & 1.6 & 1.9 \\
\midrule
Mistral~7B~v0.1\\
\midrule
Embed v3 & 46.9 & 48.5 & 48.7 & 36.3 & \bf 38.3 & 37.9 & 3.4 & 4.8 & \bf 5.6 & 3.0 & \bf 3.3 & \bf 3.8 \\
E5 & \bf 47.7 & 48.5 & 49.0 & 36.3 & 37.6 & 37.9 & 3.4 & 4.5 & 5.1 & 2.8 & 3.2 & 3.5 \\
LaBSE & 47.3 & 48.5 & 49.1 & \bf 36.7 & 37.9 & \bf 38.2 & 3.3 & 4.5 & 5.3 & \bf 3.3 & 3.3 & 3.6 \\
LASER2 & 47.6 & \bf 48.7 & \bf 49.2 & 36.3 & 38.0 & 38.0 & 2.8 & 3.8 & 4.3 & 3.0 & 2.9 & 3.0 \\
SONAR & 47.2 & 48.6 & 48.4 & 36.5 & 38.1 & 37.9 & \bf 3.4 & \bf 4.9 & 5.5 & 3.4 & 3.6 & 4.0 \\
Random & 47.2 & 48.0 & 48.4 & 36.1 & 37.3 & 37.5 & 2.8 & 2.8 & 2.9 & 2.4 & 2.3 & 2.7 \\
\midrule
LLaMA~2~7B \\
\midrule
Embed v3 & 44.5 & 45.6 & \bf 46.2 & 34.5 & 35.4 & 35.9 & 2.9 & 4.0 & 4.2 & 2.2 & 3.2 & 3.3 \\
E5 & 44.7 & 45.6 & 46.1 & 34.3 & 35.3 & 35.8 & 2.7 & 4.0 & 4.2 & 1.6 & 2.9 & 3.0 \\
LaBSE & 44.6 & 45.7 & 46.1 & 34.6 & 35.6 & 35.6 & 3.0 & 4.0 & 4.3 & 2.5 & 3.5 & 3.5 \\
LASER2 & \bf 44.7 & \bf 45.9 & 46.0 & \bf 34.6 & \bf 35.7 & \bf 35.9 & 3.0 & 3.5 & 3.5 & 2.4 & 3.1 & 3.2 \\
SONAR & 44.7 & 45.6 & 46.1 & 34.4 & 35.8 & 35.9 & \bf 3.2 & \bf 4.5 & \bf 4.6 & \bf 2.5 & \bf 3.8 & \bf 3.9 \\
Random & 44.6 & 45.2 & 45.4 & 34.1 & 35.2 & 35.5 & 2.4 & 2.8 & 2.8 & 1.3 & 2.1 & 2.3 \\
\midrule
Gemma~7B \\
\midrule
Embed v3 & 52.1 & 52.9 & 53.2 & 41.8 & 42.8 & 42.7 & 26.6 & 28.0 & 28.4 & 2.0 & 3.1 & 3.8 \\
E5 & \bf 52.5 & 53.1 & 53.0 & \bf 42.1 & 42.6 & 42.8 & 26.3 & 28.0 & 28.5 & 2.0 & 2.9 & 3.3 \\
LaBSE & 52.0 & \bf 53.4 & 53.0 & 42.0 & 42.8 & 42.8 & \bf 26.7 & 28.2 & 28.8 & 2.1 & 2.9 & 3.3 \\
LASER2 & 52.2 & 53.1 & \bf 53.5 & 41.7 & 42.5 & \bf 42.9 & 26.4 & 27.5 & 28.0 & 1.9 & 2.9 & 3.2 \\
SONAR & 52.3 & 53.0 & 53.3 & 42.0 & \bf 43.0 & 42.8 & 26.6 & \bf 28.3 & \bf 28.9 & \bf 2.2 & \bf 3.4 & \bf 3.9 \\
Random & 52.0 & 52.8 & 53.0 & 41.8 & 42.4 & 42.5 & 25.8 & 26.7 & 27.0 & 1.4 & 2.0 & 2.4 \\
\bottomrule
\end{tabular}
%}
\end{center}
\caption{Benchmarking of example retrieval in $\textit{source-to-target}$ with different sentence embeddings in $k$-shot ($k \in \{1, 5, 10\}$). We report the BLEU scores for 3 LLMs (BLOOM~7B1, Mistral~7B and Gemma~7B).}
\label{tab:bleu-se-s2t}
\end{table*}

\begin{table*}[ht]
%\tiny
\centering\small
\begin{center}
%\resizebox{0.5\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
\toprule
\multicolumn{1}{c}{\bf }  & \multicolumn{3}{c}{\bf eng $\rightarrow$ fra} & \multicolumn{3}{c}{\bf eng $\rightarrow$ deu} & \multicolumn{3}{c}{\bf eng $\rightarrow$ swh} & \multicolumn{3}{c}{\bf eng $\rightarrow$ wol}\\
 {} & 1 & 5 & 10 & 1 & 5 & 10 & 1 & 5 & 10 & 1 & 5 & 10\\
\midrule
BLOOM~7B1 \\
\midrule
Embed v3 & \bf 84.9 & 86.7 & \bf 86.8 & \bf 59.5 & \bf 60.9 & 61.5 & \bf 64.7 & \bf 69.5 & 69.7 & 51.2 & 51.4 & 51.8 \\
E5 & 84.7 & 86.5 & 86.6 & 58.7 & 60.7 & 60.9 & 65.0 & 68.8 & 69.8 & 51.1 & 51.0 & 51.3 \\
LaBSE & 84.7 & 86.6 & 86.6 & 59.0 & 60.6 & 61.0 & 64.6 & 69.5 & \bf 70.1 & 49.8 & 49.6 & 50.3 \\
LASER2 & 84.7 & \bf 86.9 & 86.7 & 59.0 & 60.4 & 60.4 & 65.2 & 68.9 & 69.2 & 52.6 & 52.0 & 52.1 \\
SONAR & 84.6 & 86.6 & 86.6 & 59.3 & 60.6 & \bf 61.8 & 64.1 & 69.1 & 69.7 & \bf 52.7 & \bf 52.4 & \bf 53.1 \\
Random & 84.3 & 86.5 & 86.6 & 58.0 & 58.5 & 58.7 & 64.0 & 67.7 & 67.9 & 49.0 & 47.3 & 48.3 \\
\midrule
Mistral~7B~v0.1\\
\midrule
Embed v3 & 86.4 & \bf 87.0 & \bf 87.0 & 84.7 & 85.9 & 85.8 & \bf 42.0 & \bf 43.2 & \bf 45.7 & 44.3 & 46.6 & 47.7 \\
E5 & \bf 86.6 & 86.7 & 87.0 & 84.5 & 85.8 & 85.8 & 41.4 & 42.9 & 43.8 & 44.4 & 46.1 & 48.1 \\
LaBSE & 86.6 & 87.0 & 87.0 & 85.0 & 85.7 & 85.9 & 40.9 & 42.0 & 44.3 & 40.8 & 43.8 & 46.0 \\
LASER2 & 86.5 & 86.9 & 87.0 & 85.1 & 85.9 & 85.9 & 39.0 & 39.7 & 40.8 & 43.0 & 45.8 & 46.6 \\
SONAR & 86.4 & 86.9 & 87.0 & 85.0 & \bf 85.9 & \bf 86.1 & 41.4 & 43.0 & 44.3 & \bf 44.9 & \bf 48.2 & \bf 48.7 \\
Random & 86.4 & 86.7 & 86.7 & 84.7 & 85.7 & 85.7 & 38.1 & 36.6 & 36.7 & 39.3 & 40.3 & 42.4 \\
\midrule
LLaMA~2~7B \\
\midrule
Embed v3 & 85.7 & 86.2 & 86.3 & 84.3 & 85.2 & \bf 85.3 & \bf 49.1 & \bf 45.7 & \bf 46.9 & 47.0 & 48.8 & 49.2 \\
E5 & 85.8 & 86.1 & 86.3 & 84.1 & 84.9 & 85.0 & 48.2 & 44.8 & 46.0 & 47.0 & 48.1 & 49.5 \\
LaBSE & 85.6 & 86.3 & 86.3 & \bf 84.5 & 85.0 & 85.3 & 47.2 & 44.6 & 46.2 & 44.6 & 45.9 & 45.9 \\
LASER2 & 85.8 & 86.1 & 86.1 & 84.4 & 85.3 & 85.2 & 44.2 & 41.3 & 42.3 & 48.6 & 48.7 & 49.0 \\
SONAR & \bf 85.8 & \bf 86.3 & \bf 86.3 & 84.3 & 85.3 & 85.2 & 48.8 & 45.2 & 46.4 & \bf 48.7 & \bf 49.8 & \bf 49.7 \\
Random & 85.6 & 85.9 & 86.0 & 84.1 & 84.9 & 85.1 & 40.2 & 37.5 & 37.9 & 44.2 & 42.2 & 43.2 \\
\midrule
Gemma~7B \\
\midrule
Embed v3 & 87.7 & 88.0 & 88.0 & 87.0 & 87.3 & 87.6 & 79.6 & \bf 80.7 & 80.8 & 40.0 & 45.1 & 48.0 \\
E5 & 87.6 & 87.9 & 88.1 & 86.7 & 87.4 & 87.6 & 79.7 & 80.5 & 80.9 & 40.6 & 44.7 & 47.6 \\
LaBSE & 87.6 & \bf 88.1 & 87.9 & 87.1 & \bf 87.6 & 87.6 & 79.4 & 80.5 & \bf 81.0 & 38.3 & 43.7 & 46.5 \\
LASER2 & 87.7 & 88.0 & \bf 88.3 & \bf 87.1 & 87.5 & 87.7 & 79.4 & 80.0 & 80.7 & 38.7 & 44.5 & 47.1 \\
SONAR & \bf 87.7 & 88.0 & 88.1 & 86.9 & 87.5 & \bf 87.7 & \bf 79.7 & 80.6 & 80.8 & \bf 41.1 & \bf 46.0 & \bf 48.9 \\
Random & 87.6 & 87.9 & 88.0 & 86.8 & 87.2 & 87.3 & 78.7 & 79.8 & 79.9 & 36.2 & 39.9 & 42.6 \\
\bottomrule
\end{tabular}
%}
\end{center}
\caption{Benchmarking of example retrieval in $\textit{source-to-target}$ with different sentence embeddings. We report the COMET scores. We work with $k \in \{1, 5, 10\}$ and 3 LLMs (BLOOM~7B1, Mistral~7B and Gemma~7B).}
\label{tab:comet-se-s2t}
\end{table*}

% BLEU 5 s2t

\begin{table*}[ht]
%\tiny
\centering\small
\begin{center}
%\resizebox{0.5\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
\toprule
\multicolumn{1}{c}{\bf }  & \multicolumn{3}{c}{\bf eng $\rightarrow$ fra} & \multicolumn{3}{c}{\bf eng $\rightarrow$ deu} & \multicolumn{3}{c}{\bf eng $\rightarrow$ swh} & \multicolumn{3}{c}{\bf eng $\rightarrow$ wol}\\
 {} & 1 & 5 & 10 & 1 & 5 & 10 & 1 & 5 & 10 & 1 & 5 & 10\\
\midrule
Gemma~2B \\
\midrule
Embed v3 & 42.1 & 43.5 & \bf 44.2 & 32.1 & 33.6 & 33.6 & 11.1 & 13.6 & 14.7 & 2.4 & 2.4 & 2.9 \\
E5 & 42.4 & 43.7 & 44.2 & 32.1 & 32.9 & 33.8 & 11.4 & 13.5 & 14.0 & 2.1 & 2.4 & 2.7 \\
LaBSE & 42.5 & 43.4 & 44.0 & 32.2 & 33.8 & 33.8 & 11.1 & 13.7 & 14.1 & 2.2 & 2.6 & 2.8 \\
LASER2 & 42.4 & 43.4 & 43.8 & \bf 32.6 & 33.5 & 33.7 & 10.8 & 12.8 & 13.0 & 2.1 & 2.3 & 2.5 \\
SONAR & \bf 42.8 & \bf 43.7 & 44.1 & 32.3 & \bf 33.8 & \bf \bf 34.0 & \bf 11.6 & \bf 14.1 & \bf 14.7 & \bf 2.7 & \bf 2.9 & \bf 2.9 \\
Random & 42.2 & 42.8 & 43.3 & 31.7 & 32.8 & 33.2 & 10.7 & 12.0 & 12.6 & 1.2 & 1.5 & 1.7 \\
\midrule
OLMo~7B \\
\midrule
Embed v3 & 35.1 & 35.8 & \bf 36.2 & 23.2 & \bf 23.9 & \bf 24.1 & 3.2 & 4.2 & \bf 4.6 & 2.6 & 2.6 & 2.8 \\
E5 & \bf 35.5 & 36.0 & 35.6 & 23.1 & 23.6 & 23.5 & 3.0 & 4.0 & 4.2 & 2.2 & 2.3 & 2.4 \\
LaBSE & 35.1 & 35.9 & 36.1 & \bf 23.6 & 23.7 & 23.8 & 3.0 & 3.8 & 4.2 & 2.3 & 2.6 & 2.7 \\
LASER2 & 35.0 & 35.6 & 35.9 & 23.2 & 23.4 & 23.7 & 2.9 & 3.5 & 3.7 & 2.4 & 2.2 & 2.3 \\
SONAR & 35.2 & \bf 36.0 & 36.0 & 23.4 & 23.6 & 23.2 & \bf 3.5 & \bf 4.2 & 4.4 & \bf 2.7 & \bf 2.8 & \bf 2.9 \\
Random & 34.9 & 35.0 & 34.9 & 22.7 & 22.9 & 22.8 & 2.3 & 2.6 & 2.6 & 1.5 & 1.5 & 1.7 \\
\midrule
LLaMA 2 13B \\
\midrule
Embed v3 & 48.8 & 49.5 & 50.1 & 38.2 & 39.1 & 39.8 & 4.2 & 5.9 & 6.4 & 2.5 & 3.0 & 3.4 \\
E5 & \bf 49.1 & 49.6 & 50.3 & 38.6 & 39.1 & 39.4 & 4.2 & 5.5 & 6.0 & 2.1 & 2.9 & 3.2 \\
LaBSE & 48.5 & 50.0 & 50.0 & 38.4 & \bf 39.6 & \bf 39.9 & 4.5 & 6.0 & 6.5 & 2.7 & 3.1 & 3.2 \\
LASER2 & 48.8 & \bf 50.0 & 50.2 & \bf 38.5 & 39.3 & 39.6 & 4.2 & 5.1 & 5.4 & 2.6 & 2.8 & 2.9 \\
SONAR & 48.8 & 49.9 & \bf 50.3 & 38.4 & 39.2 & 39.7 & \bf 4.5 & \bf 6.4 & \bf 6.8 & \bf 2.8 & \bf 3.4 & \bf 3.7 \\
Random & 48.7 & 49.6 & 50.2 & 38.0 & 39.0 & 39.4 & 3.8 & 4.3 & 4.5 & 1.7 & 2.0 & 2.2 \\
\midrule
LLaMA 2 70B \\
\midrule
Embed v3 & 52.9 & 53.6 & 54.1 & 43.0 & 43.8 & 44.1 & 8.8 & 11.4 & 12.1 & 2.7 & 3.6 & 3.9 \\
E5 & 52.8 & 53.7 & 54.0 & 43.1 & 43.9 & 44.0 & 8.3 & 11.4 & 12.1 & 2.4 & 3.3 & 3.7 \\
LaBSE & \bf 53.0 & \bf 54.0 & \bf 54.2 & \bf 43.4 & 43.8 & 44.1 & \bf 9.0 & 11.4 & 12.4 & 2.7 & 3.5 & 3.8 \\
LASER2 & 52.8 & 53.9 & 54.1 & 43.1 & 44.1 & 44.1 & 8.4 & 10.1 & 11.2 & 2.6 & 3.3 & 3.4 \\
SONAR & 52.8 & 53.7 & 54.2 & 43.2 & \bf 44.2 & \bf 44.2 & 8.8 & \bf 11.5 & \bf 12.8 & \bf 3.1 & \bf 3.8 & \bf 4.1 \\
Random & 52.5 & 53.5 & 53.9 & 43.1 & 43.6 & 43.8 & 7.6 & 9.3 & 9.6 & 2.1 & 2.4 & 2.6 \\
\midrule
Mixtral~8x7B~v0.1 \\
\midrule
Embed v3 & 54.2 & 54.9 & 55.0 & 44.3 & \bf 45.3 & \bf 45.3 & 7.5 & 9.1 & 10.3 & 2.7 & 3.3 & 3.7 \\
E5 & 54.2 & 55.1 & 54.8 & 44.0 & 44.6 & 44.9 & 7.2 & 9.0 & 10.1 & 2.5 & 3.2 & 3.4 \\
LaBSE & \bf 54.5 & 54.6 & 55.2 & 44.0 & 45.1 & 45.0 & 7.4 & 8.9 & 9.9 & 2.7 & 3.2 & 3.5 \\
LASER2 & 54.4 & 55.0 & 55.5 & \bf 44.4 & 45.2 & 45.0 & 7.2 & 8.2 & 9.0 & 2.6 & 3.0 & 3.1 \\
SONAR & 54.3 & \bf 55.1 & \bf 55.1 & 44.1 & 44.9 & 45.0 & \bf 7.8 & \bf 9.4 & \bf 10.3 & \bf 2.9 & \bf 3.7 & \bf 3.8 \\
Random & 54.1 & 54.6 & 54.9 & 43.8 & 44.6 & 44.9 & 6.5 & 7.0 & 7.5 & 1.9 & 2.2 & 2.5 \\
\bottomrule
\end{tabular}
%}
\end{center}
\caption{Benchmarking of example retrieval \textit{source-to-target} with different sentence embeddings in $k$-shot ($k \in \{1, 5, 10\}$). We report the BLEU scores.}
\label{tab:more-bleu-se-s2t}
\end{table*}

% COMET 5 s2t

\begin{table*}[ht]
%\tiny
\centering\small
\begin{center}
%\resizebox{0.5\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
\toprule
\multicolumn{1}{c}{\bf }  & \multicolumn{3}{c}{\bf eng $\rightarrow$ fra} & \multicolumn{3}{c}{\bf eng $\rightarrow$ deu} & \multicolumn{3}{c}{\bf eng $\rightarrow$ swh} & \multicolumn{3}{c}{\bf eng $\rightarrow$ wol}\\
 {} & 1 & 5 & 10 & 1 & 5 & 10 & 1 & 5 & 10 & 1 & 5 & 10\\
\midrule
Gemma~2B \\
\midrule
Embed v3 & 84.8 & 85.1 & 85.4 & \bf 82.8 & 83.2 & 83.2 & 65.2 & 67.5 & \bf 69.2 & 43.5 & 45.6 & 47.3 \\
E5 & \bf 84.9 & 85.1 & 85.3 & 82.4 & 82.9 & 83.1 & 64.8 & 67.4 & 68.7 & 43.6 & 45.7 & 47.4 \\
LaBSE & 84.8 & 85.1 & 85.2 & 82.7 & 83.4 & \bf 83.6 & 64.9 & 67.8 & 68.2 & 40.3 & 43.2 & 44.1 \\
LASER2 & 84.7 & 85.1 & 85.2 & 82.6 & 83.2 & 83.4 & 64.0 & 66.8 & 66.9 & 43.1 & 45.2 & 46.5 \\
SONAR & 84.7 & \bf 85.3 & \bf 85.4 & 82.7 & \bf 83.5 & 83.4 & \bf 65.3 & \bf 68.0 & 68.9 & \bf 44.0 & \bf 47.6 & \bf 48.3 \\
Random & 84.6 & 84.7 & 85.0 & 82.3 & 82.9 & 83.1 & 63.6 & 65.3 & 65.8 & 38.2 & 39.3 & 40.4 \\
\midrule
OLMo~7B \\
\midrule
Embed v3 & 81.1 & 81.3 & 81.3 & 75.3 & 75.9 & 75.9 & 44.4 & \bf 44.1 & \bf 45.0 & 44.9 & 44.0 & 45.2 \\
E5 & 81.0 & \bf 81.6 & \bf 81.4 & 75.2 & 76.0 & 75.9 & 43.7 & 43.5 & 44.4 & 45.3 & 43.4 & 44.3 \\
LaBSE & 81.1 & 81.3 & 81.4 & 75.3 & \bf 76.2 & \bf 76.1 & 43.4 & 43.0 & 44.4 & 41.6 & 42.3 & 43.5 \\
LASER2 & 81.0 & 81.5 & 81.3 & 75.3 & 75.9 & 76.1 & 41.1 & 41.1 & 41.9 & 43.6 & 43.0 & 43.2 \\
SONAR & \bf 81.2 & 81.2 & 81.1 & \bf 75.6 & 75.9 & 76.0 & \bf 45.2 & 43.7 & 44.6 & \bf 45.6 & \bf 45.6 & \bf 45.5 \\
Random & 81.1 & 81.0 & 80.9 & 75.1 & 75.7 & 75.6 & 38.3 & 38.4 & 38.4 & 39.9 & 38.7 & 40.1 \\
\midrule
LLaMA 2 13B \\
\midrule
Embed v3 & \bf 87.2 & 87.3 & \bf 87.6 & 86.1 & 86.2 & 86.6 & 45.2 & 48.1 & 49.5 & 45.6 & 46.0 & 45.7 \\
E5 & 87.1 & 87.0 & 87.3 & 85.8 & 86.2 & 86.5 & 45.2 & 47.9 & 49.0 & 45.6 & 45.6 & 46.0 \\
LaBSE & 87.1 & \bf 87.4 & 87.5 & \bf 86.3 & \bf 86.6 & \bf 86.7 & 45.2 & 47.9 & 49.1 & 42.9 & 44.7 & 44.6 \\
LASER2 & 87.2 & 87.3 & 87.5 & 86.2 & 86.5 & 86.6 & 43.4 & 45.5 & 46.3 & 44.2 & 44.2 & 44.2 \\
SONAR & 87.2 & 87.1 & 87.5 & 86.0 & 86.2 & 86.5 & \bf 46.0 & \bf 48.6 & \bf 49.9 & \bf 46.9 & \bf 46.9 & \bf 47.3 \\
Random & 87.0 & 87.2 & 87.4 & 85.9 & 86.1 & 86.4 & 41.8 & 42.6 & 43.1 & 40.0 & 40.0 & 40.7 \\
\midrule
LLaMA 2 70B \\
\midrule
Embed v3 & 87.7 & 88.2 & 88.2 & 87.2 & 87.5 & 87.9 & \bf 56.3 & \bf 61.3 & 62.5 & 45.2 & 48.5 & 49.1 \\
E5 & 87.8 & 88.1 & 88.3 & 87.1 & 87.6 & 87.7 & 55.8 & 60.8 & 62.5 & 44.9 & 48.7 & 49.5 \\
LaBSE & \bf 87.9 & 88.2 & 88.3 & 87.4 & 87.6 & 87.7 & 56.4 & 60.6 & 62.4 & 43.3 & 47.0 & 48.1 \\
LASER2 & 87.7 & \bf 88.3 & 88.3 & \bf 87.4 & \bf 87.8 & \bf 87.9 & 54.9 & 59.1 & 60.1 & 45.5 & 48.1 & 48.0 \\
SONAR & 87.8 & 88.2 & \bf 88.4 & 87.3 & 87.6 & 87.7 & 56.0 & 61.8 & \bf 63.0 & \bf 46.6 & \bf 49.9 & \bf 50.5 \\
Random & 87.6 & 88.0 & 88.1 & 87.2 & 87.5 & 87.7 & 53.5 & 56.8 & 57.6 & 41.0 & 43.0 & 44.0 \\
\midrule
Mixtral~8x7B~v0.1 \\
\midrule
Embed v3 & 88.3 & 88.4 & 88.5 & 87.7 & 88.1 & 88.3 & \bf 55.1 & 58.2 & 60.0 & 42.8 & 48.3 & 49.9 \\
E5 & 88.2 & 88.4 & 88.4 & 87.5 & 88.1 & 88.1 & 54.2 & 57.1 & 59.4 & 41.6 & 47.5 & 49.0 \\
LaBSE & 88.3 & 88.4 & 88.5 & 87.8 & 88.1 & 88.1 & 54.8 & 57.3 & 59.3 & 40.4 & 45.7 & 47.7 \\
LASER2 & 88.0 & 88.4 & 88.6 & \bf 87.8 & \bf 88.1 & 88.2 & 53.9 & 56.0 & 57.3 & 41.6 & 46.7 & 47.6 \\
SONAR & \bf 88.3 & \bf 88.5 & \bf 88.6 & 87.7 & 88.1 & 88.3 & 55.0 & \bf 58.2 & \bf 60.1 & \bf 43.7 & \bf 49.2 & \bf 50.1 \\
Random & 88.1 & 88.3 & 88.4 & 87.6 & 88.0 & 88.1 & 52.5 & 53.5 & 54.4 & 38.7 & 42.6 & 44.6 \\
\bottomrule
\end{tabular}
%}
\end{center}
\caption{Benchmarking of example retrieval \textit{source-to-target} with different sentence embeddings in $k$-shot ($k \in \{1, 5, 10\}$). We report the COMET scores for 5 LLMs (Gemma~2B, OLMo~7B, LLaMA~2~7B, LLaMA 2 13B and Mixtral~8x7B~v0.1).}
\label{tab:more-comet-se-s2t}
\end{table*}



\subsection{Best of both worlds} \label{best_of_both_worlds}

In Section~\ref{scalability} and Appendix~\ref{appendix:scalability}, we proved the positive impact of example retrieval at different scales across multiple LLMs. Our findings indicated that BM25 is slightly better than SONAR when we evaluate with BLEU. However, SONAR significantly outperforms BM25 in terms of laCOMET. In this additional experiment, we explored whether combining the advantages of BM25 and SONAR could result in a stronger retriever in terms of both BLEU and laCOMET. We considered two possible approaches: creating a new similarity metric combining BM25 scores and SONAR cosine similarity, or their top-$k$ results. We chose the latter approach for its simplicity and intuitiveness. In this approach, given $S_{bm25} = \{x_1, \ldots , x_k\}$ (the top-$k$ examples retrieved from $\mathcal{P}$ by BM25 with a given query) and $S_{SONAR} = \{y_1, \ldots, y_k\}$ (the top-$k$ examples retrieved from $\mathcal{P}$ by SONAR with a given query), we used Borda's voting method to assign a score to each element of $S_{BM25} \cup S_{SONAR}$. If an element appeared in both sets, we incremented its score by one. The final top-$k$ examples were obtained by sorting $S_{BM25} \cup S_{SONAR}$ based on their score and selecting the top-$k$ examples with the highest score. In cases of equality between an example from $S_{SONAR}$ and an example from $S_{BM25}$, the example from $S_{SONAR}$ was ranked higher. The resulting retriever was denoted $SONAR \odot bm25$. Figure~\ref{fig:both} shows the results obtained by merging both strategies on the direction eng$\rightarrow$swh. We observe that the merged retriever obtains a higher BLEU than both of the retrievers used separately. Moreover, it is on par with SONAR when it comes to laCOMET with a few exceptions (BLOOM~7B1, OLMo~7B).


\begin{figure*}[ht]
     \centering
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=0.85\textwidth]{imgs/bleu_both.pdf}
         %\caption{$y=x$}
         %\label{fig:bleu}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=0.85\textwidth]{imgs/lacomet_both.pdf}
         %\label{fig:lacomet}
     \end{subfigure}
     \hfill
        \caption{Comparison at scale (top: BLEU, bottom: laCOMET) of example retrieval with SONAR and BM25 and their merged retriever SONAR$\odot$bm25 for eng$\rightarrow$swh in $k$-shot settings ($k \in \{1, 2, 5, 10, 20\}$).}
        \label{fig:both}
\end{figure*}

\subsection{Scalability of example retrieval via similarity search} \label{appendix:scalability}

In addition to Figure~\ref{fig:compare}, Figure~\ref{fig:compare-bleu} illustrates the superiority of example retrieval with SONAR and BM25 over random sampling in terms of BLEU scores. Interestingly, BM25 achieves higher BLEU scores compared to SONAR, which we attribute to the fact that both BLEU and BM25 operate at the $n$-gram level. Furthermore, Figure~\ref{fig:compare-fra} extends the analysis to the translation direction eng$\rightarrow$fra. Here, example retrieval with SONAR exhibits better laCOMET scores, and the advantage of BLEU scores with BM25 becomes less pronounced.

\begin{figure*}[ht]
     \centering
     \includegraphics[width=\textwidth]{imgs/bleu.pdf}
    \caption{BLEU scores of example retrieval with SONAR, BM25 and random sampling under various selection pool constitutions for BLOOM~7B1 and eng$\rightarrow$swh in $k$-shot settings ($k \in \{1, 5, 10\}$). The big star corresponds to initial pool, that is the FLORES-200 dev set.}
    \label{fig:compare-bleu}
\end{figure*}

\begin{figure*}[ht]
     \centering
     \begin{subfigure}{\textwidth}
         \centering
         \includegraphics[width=0.85\textwidth]{imgs/bleu_fra.pdf}
         %\caption{$y=x$}
         %\label{fig:bleu}
     \end{subfigure}
     \hfill
     \begin{subfigure}{\textwidth}
         \centering
         \includegraphics[width=0.85\textwidth]{imgs/lacomet_fra.pdf}
         %\caption{$y=3\sin x$}
         %\label{fig:lacomet}
     \end{subfigure}
     \hfill
    \caption{Performance of example retrieval (top: BLEU, bottom: laCOMET) in $k$-shot settings ($k \in \{1, 2, 5, 10, 20\}$).}
    \label{fig:compare-fra}
\end{figure*}


\subsection{Robustness to the quality and the diversity of the selection pool for eng$\rightarrow$fra} \label{appendix:robustness}

%In addition to Figure~\ref{fig:robustness-lacomet}, Figure~\ref{fig:robustness-bleu} illustrates how example retrieval is influenced by the composition of the pool in terms of BLEU scores. 
Figure~\ref{fig:robustness-fra-both} presents a similar analysis with BLEU and laCOMET for the translation direction eng$\rightarrow$fra. The findings are the same as those of the eng$\rightarrow$swh direction provided in Section~\ref{robustness}, indicating that example retrieval with SONAR is the most robust approach to noisy samples.

\begin{figure*}[ht]
     \centering
     \includegraphics[width=\textwidth]{imgs/robustness_bleu.pdf}
    \caption{BLEU scores of example retrieval with SONAR, BM25 and Random sampling under various selection pool constitutions in $k$-shot, $k \in \{1, 5, 10\}$. The translation direction is eng$\rightarrow$swh and we work with BLOOM~7B1. The big star corresponds to initial pool, that is the FLORES-200 dev set.}
    \label{fig:robustness-bleu}
\end{figure*}

\begin{figure*}[ht]
     \centering
     \begin{subfigure}{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{imgs/robustness_bleu_fra.pdf}
         %\caption{$y=x$}
         %\label{fig:bleu}
     \end{subfigure}
     \hfill
     \begin{subfigure}{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{imgs/robustness_lacomet_fra.pdf}
         %\caption{$y=3\sin x$}
         %\label{fig:lacomet}
     \end{subfigure}
     \hfill
        \caption{BLEU (top) and laCOMET (bottom) scores of example retrieval with SONAR, BM25 and random sampling under various selection pool compositions. We consider the direction eng$\rightarrow$fra in $k$-shot ($k \in \{1, 5, 10\}$) and BLOOM~7B1. The big star corresponds to initial pool, that is the FLORES-200 dev set.}
        \label{fig:robustness-fra-both}
\end{figure*}
